Active Listener: Continuous Generation of Listener's Head Motion Response in Dyadic Interactions

A key component of dyadic spoken interactions is the contextually relevant non-verbal gestures, such as head movements that reflect a listener's response to the interlocutor's speech. Although significant progress has been made in the context of generating co-speech gestures, generating listener's response has remained a challenge. We introduce the task of generating continuous head motion response of a listener in response to the speaker's speech in real time. To this end, we propose a graph-based end-to-end crossmodal model that takes interlocutor's speech audio as input and directly generates head pose angles (roll, pitch, yaw) of the listener in real time. Different from previous work, our approach is completely data-driven, does not require manual annotations or oversimplify head motion to merely nods and shakes. Extensive evaluation on the dyadic interaction sessions on the IEMOCAP dataset shows that our model produces a low overall error (4.5 degrees) and a high frame rate, thereby indicating its deployability in real-world human-robot interaction systems. Our code is available at - https://github.com/bigzen/Active-Listener

==> tables/speed.tex <==
\caption{Speed of head pose generation for best case models}
\label{tab:fps}
\centering
\begin{tabular}{c|c c}
\toprule
\bf  & {\bf Speed} (in \textit{fps}) & Model size\\
\midrule
LSTM     &  1408.89 & 1.5M\\
\bf Ours  &  1450.21 & 3.32M\\
\bottomrule
\end{tabular}

==> tables/sym.tex <==
\caption{Results of speaker independent model}
\label{tab:results_main}
\centering
\begin{tabular}{l |ccc|ccc| ccc}
    \hline
    \bf Model & \multicolumn{3}{c}{\bf ROLL} & \multicolumn{3}{c}{\bf PITCH} & \multicolumn{3}{c}{\bf YAW} \\
      & \bf MAE & \bf CC & \bf p-val & \bf MAE & \bf CC & \bf p-val & \bf MAE & \bf CC & \bf p-val\\
    \hline
                    LSTM & $6.17\pm2.91$ & $0.14$ & $0.07$ & $6.41\pm3.20$ & $0.15$ & $0.08$ & $6.46\pm3.16$ & $0.13$ & $0.08$\\
                   graph & $3.27\pm2.91$ & $0.05$ & $0.24$ & $3.87\pm2.07$ & $0.01$ & $0.24$ & $6.10\pm5.06$ & $0.08$ & $0.20$\\
    \hline
\end{tabular}


==> tables/valence.tex <==
\caption{Effect of Speaker's affect on listener's reaction}
\label{tab:val}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\bf Roll} & \multicolumn{2}{c|}{\bf Pitch} & \multicolumn{2}{c|}{\bf Yaw}\\
\hline
\bf MAE & \bf CC &\bf MAE & \bf CC &\bf MAE & \bf CC\\
\hline
$3.12\pm3.58$ & $0.02$ & $3.35\pm2.67$ & $0.005$ & $6.39\pm5.48$ & $0.036$\\
\hline
\end{tabular}
